Machine Learning for Improved Current Density Reconstruction from 2D Vector Magnetic Images

The reconstruction of electrical current densities from magnetic field measurements is an important technique with applications in materials science, circuit design, quality control, plasma physics, and biology. Analytic reconstruction methods exist for planar currents, but break down in the presence of high spatial frequency noise or large standoff distance, restricting the types of systems that can be studied. Here, we demonstrate the use of a deep convolutional neural network for current density reconstruction from two-dimensional (2D) images of vector magnetic fields acquired by a quantum diamond microscope (QDM) utilizing a surface layer of Nitrogen Vacancy (NV) centers in diamond. Trained network performance significantly exceeds analytic reconstruction for data with high noise or large standoff distances. This machine learning technique can perform quality inversions on lower SNR data, reducing the data collection time by a factor of about 400 and permitting reconstructions of weaker and three-dimensional current sources.

==> introduction.tex <==
\section{Introduction}

The study of electric current distributions through imaging of Oersted magnetic fields has supported applications in many areas of physics, engineering, and medicine, in part due to its non-invasive nature \cite{orozco_magnetic_2009}.  Such applications include assessment of integrated circuits \cite{orozco_magnetic_2009, nowodzinski_nitrogen-vacancy_2015,infante_new_2009,levine_backside_2020,kehayias_measurement_2022,turner_quantum_2020,turner_magnetic_2020}, microelectronics \cite{infante_magnetic_2009,oliver_vector_2021,felt_construction_2007}, batteries \cite{hu_battery_2019,hu_sensitive_2020,bason_non-invasive_2022,brauchle_direct_2021}, solar panels \cite{scholten_imaging_2022,kaufmann_evaluation_2021}, superconducting tape and wires \cite{chikumoto_characterization_2021,sakai_effect_2023}, mechanical joints \cite{bevington_non-destructive_2018}, fault analysis \cite{wikswo_magnetic_1996}, superconducting materials and qubits \cite{wu_characterization_2021,kirtley_fundamental_2010,marchiori_magnetic_2022}, exotic materials \cite{ku_imaging_2020, feng_helical_2022,palm_imaging_2022,bjorlig_current_2022}, new semiconductor technology \cite{basso_electric_2023,lillie_imaging_2019}, and eddy current imaging \cite{wickenbrock_eddy_2016}. In medicine, imaging of magnetic fields generated by currents in biological tissues allows detailed and unique study of the heart, brain, and skeletal muscles \cite{roth_biomagnetism_2023,leder_noninvasive_1998,merwa_solution_2005,hamalainen_magnetoencephalography---theory_1993, alvarez_biomagnetic_1990, knappe_microfabricated_2016,limes_portable_2020}.

To enable these studies, current density distributions confined to thin planes are traditionally calculated utilizing Fourier space relationships between the source current density and the measured magnetic field.  Despite its widespread usage, this ``Fourier Method" for the magnetic inverse problem (i.e. the current density reconstruction problem) cannot effectively address high-noise measurements \cite{roth_using_1989}; it also performs poorly when the standoff distance between the measured magnetic field and the source current density is greater than the feature size of the current distribution. Due to these limitations, the Fourier Method sometimes results in poor analytic reconstructions \cite{turner_magnetic_2020, roth_using_1989}.  These drawbacks most heavily impact its utility for systems with small features or restricted standoff distance, such as nondestructive quality control and failure analysis of intact semiconductor chips, imaging of wires through walls or device boundaries, and noninvasive measurements of biological systems, which commonly exhibit weak magnetic field signals and small, irregular features \cite{roth_biomagnetism_2023}.

Due to the poor reconstruction performance of the Fourier Method in the low 
signal-to-noise-ratio (SNR) regime and/or at large standoff distance, many repeated magnetic field measurements are typically required to achieve sufficient SNR, significantly slowing the measurement process and leading to systematic errors related to drift in the measured system or instrumentation \cite{levine_principles_2019}. An alternative current reconstruction technique requiring fewer measurements could enable higher fidelity results, the study of dynamic processes in samples that would otherwise be immeasurable, and greatly increase the speed of device quality control applications.

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{fig1.pdf}
    \caption{(a) Illustration of the training process. The MAGIC-UNet network is trained on field-current pairs, taking inputs of vector magnetic field images and making predictions of planar current density distributions. After each batch, the predicted currents are compared to the ground truth using mean squared error; and then network weights are updated to improve the accuracy of the prediction. After many iterations the network will have learned to make quality predictions for unknown currents. (b) Diagram showing the structure of the MAGIC-UNet network. Colored blocks represent different layers or groups of layers. Downsampling uses a 2x2 average pooling layer; upsampling also includes a 3x3 convolutional layer. Concatenation is represented by a $\framebox{C}$  symbol and allows skip connections to join inputs from earlier parts of the network to later stages. The network has a branched structure with separate paths for $J_x$ and $J_y$, which do not interact.}
    \label{schematic}
\end{figure*}
\noindent

Neural networks excel at tackling a variety of image-based inverse problems \cite{jin_deep_2017,wang2020deep,schlemper2019dautomap,zhu_image_2018}. While early attempts at applying neural networks to the magnetic inverse problem operated in highly restricted parameter spaces \cite{coccorese_neural_1994,kishimoto_solution_1996}, advances in computing power and machine learning techniques show promise for identification of current density features of unrestricted sizes, shapes, and strengths in noisy images \cite{mccann_convolutional_2017}. In particular, convolutional Neural Networks, including UNets \cite{ronneberger_u-net_2015} have shown impressive results in medical imaging reconstruction problems with regard to de-noising and artifact reduction  \cite{mehta2022mri,chen2017low}; and more generally in preserving structural features \cite{jin_deep_2017}.  In addition to UNet performance benefits, the lack of fully connected layers allows for training with higher resolution inputs and the ability to use a single network for multiple image sizes.

In this work, we present an adapted UNet architecture (MAGnetic Inverse Calculation UNet) designed for reconstructing current density images from vector magnetic field images with greater accuracy than the Fourier Method. The MAGIC-UNet network is tested on a variety of synthetic data types and experimentally collected Oersted magnetic field images using a Quantum Diamond Microscope (QDM). The QDM utilizes a dense, near-surface layer of nitrogen vacancy (NV) quantum defects in a diamond substrate to enable sensitive magnetic imaging, with micron-scale spatial resolution, via optical emission of the NV defects \cite{levine_principles_2019}. The MAGIC-UNet network is trained, in less than twelve hours, on hundreds of thousands of field-current image pairs generated analytically through Biot-Savart forward calculations of vector magnetic fields from randomly generated planar current density distributions (Figure \ref{schematic}a). We present current density reconstructions from both simulations and QDM experiments utilizing the MAGIC-UNet network, demonstrating greatly enhanced performance compared to the Fourier Method, and reliable reconstructions even in the presence of extreme noise (input SNR $\sim$ 1).
